Non-Parametric Cluster Significance Testing with Reference to a Unimodal Null Distribution

Cluster analysis is an unsupervised learning strategy that can be employed to identify subgroups of observations in data sets of unknown structure. This strategy is particularly useful for analyzing high-dimensional data such as microarray gene expression data. Many clustering methods are available, but it is challenging to determine if the identified clusters represent distinct subgroups. We propose a novel strategy to investigate the significance of identified clusters by comparing the within- cluster sum of squares from the original data to that produced by clustering an appropriate unimodal null distribution. The null distribution we present for this problem uses kernel density estimation and thus does not require that the data follow any particular distribution. We find that our method can accurately test for the presence of clustering even when the number of features is high.

==> ArXiv submission/theory_abv_JASA.tex <==
 We now seek to establish several important theoretical properties for our reference distribution and cluster index test statistic. \citet{tibshirani2001estimating} show that for their gap statistic, a statistic also based on the sum of squares, that there is no least favorable multivariate unimodal reference distribution without degenerate support. Also they state that a maximum likelihood estimate of a multivariate unimodal reference distribution can not be shown to exist. Thus we we will not be able to choose a generally applicable reference distribution. However we can show that our reference distribution has optimal characteristics such as convergence in first and second moments and multivariate unimodality. We also seek to show asymptotic convergence of the CI from the reference distribution to the data CI when the data in unclustered and asymptotic divergence when the data is clustered.

  When $n>p$ it is trivial to show that the first and second moments of our proposed reference distribution asymptotically approach the first and second moments of the observed data. When $p>n$ showing the convergence of second moment depends on the method used to estimate the covariance (in this paper the graphical lasso is used)  and is beyond the scope of this paper. 
   
   From \citet{Silverman1981using} we have that $ h_{1j}$ can be chosen such that $\hat{f}(\dot,h_{1j})$ has at most one mode. Thus before multiplying by the Cholesky root each feature in our reference distribution is unimodal. To show that the marginal distributions retain their unimodality and the joint reference distribution is multivariate unimodal we appeal to the concept of \textit{strong unimodality}. \citet{Ibragimov1956on} defines a distribution function to be $\emph{strong unimodal}$ if its composition with any unimodal distribution function is unimodal. We show that the features are strong unimodal and thus the final marginal distributions are unimodal. 
   \\
   
      \textit{Theorem 1}. Each feature in the reference distribution is strong unimodal. 
      \\
      
  We now need to show that our transformed distribution is multivariate unimodal. To do so we will use the definition 2.5 from \citet{Sager1978Estimation}. Let $\boldsymbol{x}$ be a point in p-space $\boldsymbol{x}=(x_1,..,x_p)$ and $d(\boldsymbol{x},\boldsymbol{y})$ be the Euclidean metric $|\boldsymbol{x}-\boldsymbol{y}|$. He defines a point $\boldsymbol{\theta}$ to be a  multivariate mode of $F$ if for each $\epsilon>0$, $\exists \ \delta >0$ s.t. $d(\boldsymbol{x},\boldsymbol{\theta})> \epsilon$ implies $f(\boldsymbol{x})$+ $\delta < f(\boldsymbol{\theta})$.
  \\
  
  \textit{Theorem 2}. Suppose that each feature $x_j$ is independent and unimodal with mode $max(f_j(x_j))=m_j$ and the unique mode for $f(x_1,..,x_p)$ is given by:  
  \begin{math}
  \underset{\boldsymbol{x}}{max} \{\ f(x_1,..,x_p) \} =<m_1,...,m_p>
  \end{math}. Then after multiplying by the Cholesky root of the covariance matrix the resulting distribution, $h(y_1,...,y_p)$, is multivariate unimodal.  
    \\
  
  We now show asymptotic convergence of our null CI to the data CI when the data is unclustered and divergence when the data is clustered. As $n \rightarrow \infty$ the sample data becomes continuous so our proof compares the theoretical cluster index, the cluster index assuming continuity in the data, from the null distribution to the theoretical distribution from the data. The theoretical cluster index is defined to be the theoretical within cluster sum of squares divided by the theoretical total sum of squares.  The within cluster sum of squares is based off of a partition of the feature space into two non-overlapping subspaces $S_1$ and $S_2$. Using the same notation as \citet{Huang2015statistical} the theoretical sum of squares is given by: 
   \begin{equation}
   TCI=\frac{WSS}{TSS}=\frac{WSS_1+WSS_2}{TSS}
   =\frac{\int_{\boldsymbol{x} \in S_1} ||\boldsymbol{x}-\boldsymbol{\mu_1}||^2\phi(x)dx +\int_{\boldsymbol{x}\in S_2} ||\boldsymbol{x}-\boldsymbol{\mu_2}||^2\phi(x) dx}{\int||\boldsymbol{x}||^2\phi(x)dx}
      \end{equation}
      Where $\boldsymbol{\mu_k}=\int_{\boldsymbol{x}\in S_k} \boldsymbol{x}\phi(x)dx$
      \\
   
   \textit{Theorem 3}.   Let $\boldsymbol{x}= (x_1,\dots, x_p)$ be a d-dimensional random vector having a multivariate normal    distribution of $ \boldsymbol{x} \sim N(\boldsymbol{0},\boldsymbol{D})$ where $\boldsymbol{D}$ is a known covariance matrix with diagonal entries $\lambda_1 \ge \lambda_2 \ge \dots \ge \lambda_p$. Let $TCI_{GAUSS}$ represent the theoretical cluster index of $\boldsymbol{x}$.  For the choice of $S_1$ and $S_2$ which minimizes WSS, \begin{math}
    TCI_{GAUSS}=1-\frac{2}{\pi}\frac{\lambda_1}{\sum_{j=1}^p\lambda_j}
    \end{math}. The theoretical cluster index for our null distribution, $TCI_{null}$ approaches $TCI_{GAUSS}$ as n $ \rightarrow \infty$.
    \\
    
     \textit{Theorem 4}.
   Let $x = (x_1,\dots, x_p)$ be a p-dimensional random vector having a mixture multivariate normal distribution. Specifically the data is distributed as $\eta f(x)+(1-\eta)g(x)$ where $f(x) \sim N(\boldsymbol{0},\boldsymbol{D})$, $g(x) \sim N(\boldsymbol{\mu},\boldsymbol{D})$,  $\eta \in (0,1)$ is the mixing proportion, $\boldsymbol{\mu}=(a,\dots,a)^T$ with nonzero constant a, and $\boldsymbol{D}$ is a diagonal matrix with elements $\lambda_1 \ge \lambda_2 \ge \dots \ge \lambda_p$. Suppose  the mixing proportion $\eta$ stays constant as $n \rightarrow \infty$. Also assume that the clustering algorithm is able to correctly classify the $n_1$ observations that arise from the $N(\boldsymbol{0},\boldsymbol{D})$ distribution into cluster 1 and the $n_2$ observations that arise from the $N(\boldsymbol{\mu},\boldsymbol{D})$ distribution into cluster 2. Let $TCI_{mix}$ represent the theoretical cluster index from the mixture distribution. Then we have that $\underset{n \rightarrow \infty }{\lim}TCI_{mix}<\underset{n \rightarrow \infty }{\lim}TCI_{null}$.
   \\
   
   Up to this point we have focused on $n \rightarrow \infty$ asymptotics for the cluster index. We now establish asymptotic properties as $p \rightarrow \infty$.
   \\
   
   \textit{Theorem 5}.
    Let $X$ be a mixture of two Gaussian distributions $X=\eta N(\boldsymbol{0},\boldsymbol{D})+ (1-\eta)N(\boldsymbol{\mu},\boldsymbol{D})$ where $X$ is an $ n \times p$ matrix and $\eta \in (0,1)$ is the mixing proportion. Let $n_1$ be the number of observations collected from $N(\boldsymbol{0},\boldsymbol{D})$ and $n_2$ be the number of observations collected from $N(\boldsymbol{\mu},\boldsymbol{D})$, Define $\boldsymbol{\mu}=(a,...,a)^T$ with a $\ne$ 0. Suppose $\boldsymbol{D}$ is a known diagonal covariance matrix with elements $\lambda_1>...>\lambda_p$. Note that the variance for feature j from the mixture distribution is given by $\lambda_j+\eta(1-\eta)a^2$. Assume n is fixed;  $min(n_1,n_2)>0$; $n_1+n_2=n \ge 3$; $\Sigma_{j=1}^p\lambda_j=O(p^\beta)$ with $0 \le \beta < 1$; $max_j(\lambda_j+\eta(1-\eta)\alpha^2) \le M$ with $M>0$ a fixed constant. Let the observed data with scaled and centered features be denoted as $X^s$. Also assume that a finite bandwidth $h_{1j}$, $max_j(h_{1j})<L$ with $L>0$ a fixed constant, can be chosen for each feature of $X^s$ such that the Gaussian kernel density estimator is unimodal. Then we can show that the corresponding p-value converges to 0 in probability as $ p \rightarrow \infty$.
